You Cannot Recover What Was Never Measured: Quantifying the Information Ceiling of Ultra-Low-Field MRI Super-Resolution

Generative super-resolution models can turn portable 64 mT MRI into images that look like 3T scans, and the field evaluates them with PSNR, SSIM, and pixelwise uncertainty, most often on pairs built by synthetically degrading high-field images. Prior work acknowledges that these models hallucinate and that the problem is ill posed, but to our knowledge no study measures how much information about the individual subject the real low-field scan actually contains. We measure it. Using paired 64 mT and 3T scans of the same subjects from three public datasets, and a measurement protocol validated on tests whose correct answer is known in advance, we find that, judged over the whole brain, real 64 mT scans carry structure specific to the individual only down to approximately 3 to 4 mm half-pitch in plane, and coarser still through plane. Standard synthetic degradations preserve subject information roughly 1 mm beyond this ceiling, so models trained and benchmarked on synthetic pairs are evaluated on information that real scanners never record. We then test trained diffusion models and a publicly released external model on real paired acquisitions; 24 trained runs of five architectures (GAN, diffusion, and transformer families) give the coverage of the audit. On every subject where faithfulness can be measured, fine output detail is no more correlated with the subject's own 3T scan than with a stranger's, while sample-variance uncertainty does not distinguish fabricated structure from reconstruction difficulty. Because PSNR and SSIM score resemblance to a reference rather than whether detail belongs to the subject, a benchmark scored by them cannot tell recovery from fabrication. Code for the measurement protocol will be released so that recoverability claims can be tested for newer models.

==> selected_results_20260924_v4/selected_results/images.tex <==

\providecommand{\selectedresultspath}{selected_results}
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{\selectedresultspath/panel_03.png}
\par\smallskip
\includegraphics[width=\textwidth]{\selectedresultspath/panel_04.png}
\par\smallskip
\caption{Matched examples A and B within each panel. Columns show low-field input (LF), high-field reference (GT) and seed-0 reconstructions; IDs refer to Table~\ref{tab:selected-metrics}. A/B are independent case labels within each panel and are not shared subjects across datasets or contrasts. Images use fixed intensity mapping without per-image contrast stretching. Display cropping/zoom is identical across columns within each panel. Multi-contrast panels reconstruct T2; LF shows the T2 input channel.}
\label{fig:selected-images-1}
\end{figure*}
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{\selectedresultspath/panel_01.png}
\par\smallskip
\includegraphics[width=\textwidth]{\selectedresultspath/panel_02.png}
\par\smallskip
\caption{Matched examples A and B within each panel. Columns show low-field input (LF), high-field reference (GT) and seed-0 reconstructions; IDs refer to Table~\ref{tab:selected-metrics}. A/B are independent case labels within each panel and are not shared subjects across datasets or contrasts. Images use fixed intensity mapping without per-image contrast stretching. Display cropping/zoom is identical across columns within each panel. NIST uses a shared rotated anatomy crop with approximately $2\times$ central display zoom.}

\label{fig:selected-images-2}
\end{figure*}
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{\selectedresultspath/panel_05.png}
\par\smallskip
\includegraphics[width=\textwidth]{\selectedresultspath/panel_06.png}
\par\smallskip
\caption{Matched examples A and B within each panel. Columns show low-field input (LF), high-field reference (GT) and seed-0 reconstructions; IDs refer to Table~\ref{tab:selected-metrics}. A/B are independent case labels within each panel and are not shared subjects across datasets or contrasts. Images use fixed intensity mapping without per-image contrast stretching. Display cropping/zoom is identical across columns within each panel. Multi-contrast panels reconstruct T2; LF shows the T2 input channel.}

\label{fig:selected-images-3}
\end{figure*}


==> selected_results_20260924_v4/selected_results/metrics.tex <==
\begin{table*}[t]
\centering\scriptsize
\caption{Reconstruction quality for the selected experiments: five-inference-seed mean and sample standard deviation.}
\label{tab:selected-metrics}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llrrrr@{}}
\toprule
Group & Experiment / setting & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NMSE $\downarrow$ \\
\midrule
Zenodo T2 & E01 Res-SRDiff / Min-Max Perceptual Wavelet & $19.40\,\pm\,0.0016$ & $0.6720\,\pm\,5.4\times10^{-5}$ & $0.1903\,\pm\,3.4\times10^{-5}$ & $\boldsymbol{0.2966\,\pm\,0.0004}$ \\
 & E02 Res-SRDiff / T2+FLAIR / Fixed-percentile Balanced & $22.28\,\pm\,0.0012$ & $0.7031\,\pm\,9.4\times10^{-6}$ & $0.2141\,\pm\,3.4\times10^{-5}$ & $0.4594\,\pm\,0.0001$ \\
 & E03 Res-SRDiff / T2+T1 / Fixed-percentile Balanced & $\boldsymbol{22.41\,\pm\,0.0024}$ & $0.7119\,\pm\,4.1\times10^{-5}$ & $0.2008\,\pm\,4.6\times10^{-5}$ & $0.4497\,\pm\,0.0002$ \\
 & E04 Res-SRDiff / T2+T1+FLAIR / Fixed-percentile Balanced & $22.39\,\pm\,0.0049$ & $\boldsymbol{0.7157\,\pm\,0.0001}$ & $\boldsymbol{0.1817\,\pm\,8.4\times10^{-5}}$ & $0.4195\,\pm\,0.0005$ \\
\midrule
Zenodo T1 & E05 Res-SRDiff / WhiteStripe Perceptual Wavelet & $\boldsymbol{18.67\,\pm\,0.0024}$ & $0.5947\,\pm\,0.0002$ & $\boldsymbol{0.1998\,\pm\,9.7\times10^{-5}}$ & $0.3252\,\pm\,0.0011$ \\
 & E06 Res-SRDiff / WhiteStripe Balanced Image & $18.40\,\pm\,0.0018$ & $0.5185\,\pm\,0.0006$ & $0.2065\,\pm\,0.0002$ & $\boldsymbol{0.3156\,\pm\,0.0006}$ \\
 & E07 Res-SRDiff / Min-Max Perceptual Wavelet & $18.08\,\pm\,0.0016$ & $\boldsymbol{0.6223\,\pm\,6.3\times10^{-5}}$ & $0.2130\,\pm\,0.0001$ & $0.3925\,\pm\,0.0008$ \\
\midrule
NIST T2 & E08 DISGAN / Min-Max Perceptual Image & $28.41\,\pm\,0$ & $0.9306\,\pm\,0$ & $0.0425\,\pm\,0$ & $0.3896\,\pm\,0$ \\
 & E09 DISGAN / WhiteStripe Balanced Image & $30.16\,\pm\,0$ & $0.8917\,\pm\,0$ & $0.0683\,\pm\,0$ & $0.3233\,\pm\,0$ \\
 & E10 medSynthesis / Min-Max Perceptual Image & $30.29\,\pm\,0$ & $0.9437\,\pm\,0$ & $0.0301\,\pm\,0$ & $0.2327\,\pm\,0$ \\
 & E11 medSynthesis / WhiteStripe Balanced Image & $32.26\,\pm\,0$ & $0.9042\,\pm\,0$ & $0.0572\,\pm\,0$ & $0.1891\,\pm\,0$ \\
 & E12 SR-CycleGAN / WhiteStripe Balanced Image & $27.59\,\pm\,0$ & $0.8800\,\pm\,0$ & $0.0769\,\pm\,0$ & $0.5371\,\pm\,0$ \\
 & E13 Res-SRDiff / Min-Max Perceptual Wavelet & $30.49\,\pm\,0.0046$ & $0.9517\,\pm\,2.3\times10^{-5}$ & $0.0363\,\pm\,1.9\times10^{-5}$ & $0.2249\,\pm\,0.0002$ \\
 & E14 Res-SRDiff / WhiteStripe Balanced Image & $32.18\,\pm\,0.0112$ & $0.9072\,\pm\,0.0001$ & $0.0572\,\pm\,7.4\times10^{-5}$ & $0.1937\,\pm\,0.0010$ \\
 & E15 Res-SRDiff / Multi-b Balanced Image & $\boldsymbol{32.73\,\pm\,0.0063}$ & $\boldsymbol{0.9629\,\pm\,2.6\times10^{-5}}$ & $\boldsymbol{0.0294\,\pm\,3.8\times10^{-5}}$ & $\boldsymbol{0.1505\,\pm\,0.0003}$ \\
 & E16 ViT & $27.68\,\pm\,0$ & $0.7682\,\pm\,0$ & -- & $6.0445\,\pm\,0$ \\
 & E17 Res-SRDiff / WhiteStripe Balanced Wavelet & $31.81\,\pm\,0.0108$ & $0.8948\,\pm\,0.0002$ & $0.0657\,\pm\,0.0001$ & $0.2082\,\pm\,0.0006$ \\
 & E18 Res-SRDiff / WhiteStripe Perceptual Wavelet & $31.43\,\pm\,0.0032$ & $0.8947\,\pm\,6.8\times10^{-5}$ & $0.0622\,\pm\,3.2\times10^{-5}$ & $0.2250\,\pm\,0.0003$ \\
\midrule
OpenNeuro T2 & E19 Res-SRDiff / Min-Max Perceptual Wavelet & $\boldsymbol{20.24\,\pm\,0.0050}$ & $\boldsymbol{0.6481\,\pm\,0.0001}$ & $\boldsymbol{0.2117\,\pm\,0.0001}$ & $0.6161\,\pm\,0.0030$ \\
 & E20 DISGAN / WhiteStripe Balanced Image & $18.36\,\pm\,0$ & $0.3872\,\pm\,0$ & $0.3325\,\pm\,0$ & $\boldsymbol{0.5732\,\pm\,0}$ \\
 & E21 medSynthesis / WhiteStripe Balanced Image & $18.27\,\pm\,0$ & $0.3841\,\pm\,0$ & $0.3415\,\pm\,0$ & $0.5740\,\pm\,0$ \\
\midrule
OpenNeuro T1 & E22 ViT / WhiteStripe & $\boldsymbol{22.11\,\pm\,0}$ & $\boldsymbol{0.7621\,\pm\,0}$ & -- & $0.9776\,\pm\,0$ \\
 & E23 DISGAN / WhiteStripe Balanced Image & $18.94\,\pm\,0$ & $0.7145\,\pm\,0$ & $\boldsymbol{0.1353\,\pm\,0}$ & $\boldsymbol{0.4225\,\pm\,0}$ \\
\bottomrule
\end{tabular}}
\par\smallskip\begin{minipage}{\textwidth}\scriptsize
Values are mean $\pm$ sample SD across five inference seeds (0--4)
of a single trained model for each row. Bold marks the best unrounded
mean per metric within each dataset/contrast block (ties: first listed
row) and is descriptive only: datasets, normalization, evaluation grids
and metric implementations differ, so it does not establish a fair
cross-dataset comparison or statistical superiority. PSNR is in dB.
-- means unrecorded. ViT is trained with global SSIM and SSIM/style
loss, not balanced GAN loss. Multi-contrast rows use fixed-percentile
scaling and reconstruct T2.\end{minipage}
\end{table*}

